Visual Foresight for Agentic Reasoning Before Action in Urban Navigation

Urban navigation requires embodied agents to pursue long-horizon goals through local decisions based on egocentric observations. However, existing agentic navigation methods often struggle to translate distant goals into coherent local decisions. Their reliance on linguistic reasoning over transient observations or limited history constrains anticipation of action consequences, despite the importance of such foresight for navigating long and complex urban routes. To bridge this gap, we propose PreAct-Nav, a training-free agentic navigation framework that equips frozen policies with visual foresight for reasoning before action. Our central idea is to use predicted future views to assess proposed actions in the context of persistent medium-horizon subgoals and observed experience. At its core, a navigation memory module maintains the active subgoal and relevant experience across decisions, translating distant goals into actionable intermediate objectives. To enable visual foresight, a predictive world sandbox uses an action-conditioned world model (AC-WM) to generate future views of proposed movements, providing visual cues for reasoning about their consequences beyond the current observation. A vision-language model (VLM) reasoner interprets these predictions using the subgoal and accumulated experience to retain or revise actions. After execution, real observations are used to assess outcomes, correct inconsistent assumptions, and update memory to continue or reformulate the subgoal. Extensive evaluations demonstrate that the proposed PreAct-Nav improves action selection through memory updates and visual prediction, with more pronounced gains on longer routes and routes with more turns.

==> table_style.tex <==
\RequirePackage{colortbl}
\definecolor{reasonergray}{gray}{0.92}
\definecolor{navgain}{RGB}{28,125,74}
\newcommand{\navgainvalue}[2]{\mbox{#1\textsuperscript{\textcolor{navgain}{#2}}}}
\newcommand{\navdelta}[1]{{\scriptsize\textcolor{navgain}{(#1)}}}
\newcommand{\navtableformat}{%
  \small
  \setlength{\tabcolsep}{4pt}%
  \renewcommand{\arraystretch}{1.08}%
}
\newcommand{\navmetrichead}{%
  \textbf{SR}$\uparrow$ & \textbf{SPL}$\uparrow$ & NE$\downarrow$ &
  nDTW$\uparrow$ & SDTW$\uparrow$ & OSR$\uparrow$%
}

